Bayesian Separation of Document Images with Hidden Markov Model

this paper we consider the problem of separating noisy instantaneous linear mixtures of document images in the Bayesian framework. The source image is modeled hierarchically by a latent labeling process representing the common classifications of document objects among different color channels and the intensity process of pixels given the class labels. A Potts Markov random field is used to model regional regularity of the classification labels inside object regions. Local dependency between neighboring pixels can also be accounted by smoothness constraint on their intensities. Within the Bayesian approach, all unknowns including the source, the classification, the mixing coefficients and the distribution parameters of these variables are estimated from their posterior laws. The corresponding Bayesian computations are done by MCMC sampling algorithm. Results from experiments on synthetic and real image mixtures are presented to illustrate the performance of the proposed method.

==> abstract.tex <==
\fontsize{9}{11}\selectfont In this paper we consider the problem of separating noisy instantaneous linear mixtures of document images in the Bayesian framework. The source image is modeled hierarchically by a latent labeling process representing the common classifications of document objects among different color channels and the intensity process of pixels given the class labels. A Potts Markov random field is used to model regional regularity of the classification labels inside object regions. Local dependency between neighboring pixels can also be accounted by smoothness constraint on their intensities. Within the Bayesian approach, all unknowns including the source, the classification, the mixing coefficients and the distribution parameters of these variables are estimated from their posterior laws. The corresponding Bayesian computations are done by MCMC sampling algorithm. Results from experiments on synthetic and real image mixtures are presented to illustrate the performance of the proposed method.


==> authors.tex <==
\author{{\textmd {\textbf }}\\
  \fontsize{11}{13}\selectfont
  Feng SU$^{\dagger\ast}$, Ali MOHAMMAD-DJAFARI$^{\dagger}$\\
  \fontsize{9}{11}\selectfont
  \textit{$^\dagger$Laboratoire des Signaux et Systemes, UMR 8506 (CNRS-Supelec-UPS)}\\
  \textit{Supelec, Plateau de Moulon, 3 rue Joliot Curie, 91192 Gif-sur-Yvette, France}\\
  \textit{$^\ast$State Key Laboratory for Novel Software Technology, Nanjing University, 210093 Nanjing, P.R.China}\\
  \fontsize{9}{11}\selectfont
  \textit{Firstname.Lastname@lss.supelec.fr}\\[12pt]
  % repeat previous group of commands here for further authors
}


==> keywords.tex <==
\fontsize{9}{11}\selectfont Blind Source Separation, document image, Bayesian estimation, HMM, MCMC.


==> title.tex <==
% The Title is all in Uppercase
\newcommand{\mytitle}{\uppercase{Bayesian Separation of Document Images with Hidden Markov Model}
%\\
% The Subtitle should have initial letters capitalized
%\fontsize{13}{15}\selectfont \textit{...Subtitle Goes Here...}
}

